Data-driven reference model selection and application to L-DDC design

The choice of a reference model in data-driven control techniques is a critical step. Indeed, it should represent the desired closed-loop performances and be achievable by the plant at the same time. In this paper, we propose a method to build such a reference model, both reproducible by the system and having a desired behaviour. It is applicable to Linear Time-Invariant (LTI) monovariable systems and relies on the estimation of the plant's instabilities through a data-driven stability analysis technique. The L-DDC (Loewner Data Driven Control) algorithm is used to illustrate the impact of the choice of the reference model on the control design process. Finally, the proposed choice of specifications allows to use a controller validation technique based on the small-gain theorem.

==> rebut.tex <==




As recalled in \cite{zhou1998essentials}, a closed-loop is internally stable if and only if the sensitivity function is stable and if there are no compensation of instabilities in the open-loop. \par Therefore, for a NMP system with a poorly chosen reference model $M$, the ideal controller $K^\star$ may destabilize the plant internally. In this case, $K^\star$ represents a terrible behaviour that should not be reproduced in the designed controller. This is contradictory with the principle of the mentioned model-reference techniques.

It is an interpolatory method initially used for model approximation and reduction. It constructs a descriptor model in state-space form directly from the frequency-domain data so that the model performs a barycentric Lagrange interpolation. The Loewner approach is also able to find the smallest exact interpolating model for a generalized realization problem.

\begin{figure*}
    \centering
    \subfloat[][Interpolation of the ideal controller $K^\star$ (order 10) using the Loewner framework, and its stable projection.] {\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 2.5cm, clip]{controleur_stable.pdf}\label{Kstab}}
    \subfloat[][Resulting closed-loops.] {\includegraphics[width=0.45\textwidth, trim=0cm 0cm 0cm 2.5cm, clip]{boucle_fermee_stab.pdf}\label{Hstab}}
    \caption{Identification of a stable controller to avoid compensation of instabilities in the open-loop.}
    \label{result_stab}
\end{figure*}

 as follows: $   \hat{A}^{as}=(J_1\mathcal{O}_{n_F})^\dagger J_2\mathcal{O}_{n_F}$,
with $J_1=\left[ I_{(n_F-1)n_p)}\ 0_{(n_F-1)n_p \times n_p}\right]$ and $J_2=\left[  0_{(n_F-1)n_p \times n_p}\ I_{(n_F-1)n_p)}\right]$. 

Finally, the estimated unstable poles of the plant $P$ are obtained by applying the inverse of the bilinear Mobius transform, see \eqref{Pf}.


Assuming that a state-space representation $\left(A^{as},B^{as},C^{as},D^{as}\right)$ of $P^{as}_{f}$ is available, the associated observability and controlability matrices, respectively denoted $\mathcal{O}^{as}$ $\mathcal{C}^{as}$ satisfy:
\begin{equation}
    \Phi_{n_F}=\mathcal{O}^{as}\mathcal{C}^{as}.
    \label{Hankel_OC}
\end{equation}
\par Following \eqref{Hankel_OC}, the observablity and controlability matrices can be approximated by: $\mathcal{O}_{n_F}=U_P\sqrt{S_P}$ and $\mathcal{C}_{n_F}=\sqrt{S_P}V_P$.
$\mathcal{O}_{n_F}$ is the extended observability matrix of $P^{as}$ and satisfies:
\begin{equation}
    \mathcal{O}_{n_F}^T=\begin{pmatrix} {C^{as}}^T & {\left(C^{as}A^{as}\right)}^T & \dots & {\left(C^{as}(A^{as})^{n_F-1}\right)}^T\end{pmatrix}.
    \label{OnF}
\end{equation}
Therefore, it is possible to estimate the matrix $A^{as}$ from $\mathcal{O}_{n_F}$. The unstable poles of $P$ are given by the eigenvalues of $\hat{A}^{as}$. 

==> rebut_annexe.tex <==
\subsection{Preliminary results: Loewner Data-Driven Control}
%When it comes to model-reference control techniques, as VRFT, CbT or L-DDC, the objective is to design a controller that minimizes the error between the resulting closed-loop and the desired one. The problem is shown on Figure \ref{problem_formulation}.

\par \leavevmode \par  The L-DDC algorithm, introduced in \cite{kergus2017}, is based on frequency-domain data $\left\{\omega_i,P(\imath\omega_i)\right\}_{i=1}^{N}$ collected from the plant. It is a one shot technique in which the order of the controller is a tunable parameter. It only requires a reference model $M$. The LDDC algorithm is recalled hereafter.
\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Solution}{Solution}
\KwData{\begin{itemize}
    \item Samples of the frequency response of the plant $\{\omega_{i},P(\imath\omega_i)\}, \ i=1 \ldots N$.
    \item Objective order $n$ for the controller.
    \item Reference transfer function $M$.
\end{itemize}}
\Solution{
\begin{enumerate}
    \item Compute the samples of the frequency response of the ideal controller according to \eqref{Kideal}.
    
    \item Using the Loewner framework, compute the interpolating descriptor controller model $K$.
    
    \item Compute its projection $K^s$ on $\mathcal{RH}_\infty$.
    
    \item Reduce $K^s$ to obtain a stable n-th order controller $K_n^s$.
    
\end{enumerate}
}
\caption{L-DDC algorithm}
\label{LDDC}
\end{algorithm}
\par \leavevmode \par  The Loewner framework allows to identify an interpolating model $K$ of the ideal controller $K^\star$ in the second step, see \cite{antoulas2015tutorial}. In order to avoid the compensation of the plant's RHP zeros, the L-DDC alorithm has been modified in \cite{kergus2018}: the interpolating model $K$ is projected on $\mathcal{RH}_\infty$, using the technique presented in \cite{kohler2014closest}. It corresponds to step 3 of Algorithm \ref{LDDC}. The reduction has also been modified in order to be more robust to noisy data. This is possible through a residue-based implementation instead of the classic SVD approach, see \cite{lefteriu2010modeling} for more information.
\par \leavevmode \par  The identification of the ideal controller in the second step makes it unnecessary to choose a structure a priori for the controller, contrary to CbT or VRFT. Despite this strength, the L-DDC technique, as the CbT and the VRFT, is confronted to the problem of choosing an achievable reference model for an unknown plant.

